P-MapNet: Far-seeing Map Generator Enhanced by both SDMap and HDMap Priors

Autonomous vehicles are gradually entering city roads today, with the help of high-definition maps (HDMaps). However, the reliance on HDMaps prevents autonomous vehicles from stepping into regions without this expensive digital infrastructure. This fact drives many researchers to study online HDMap generation algorithms, but the performance of these algorithms at far regions is still unsatisfying. We present P-MapNet, in which the letter P highlights the fact that we focus on incorporating map priors to improve model performance. Specifically, we exploit priors in both SDMap and HDMap. On one hand, we extract weakly aligned SDMap from OpenStreetMap, and encode it as an additional conditioning branch. Despite the misalignment challenge, our attention-based architecture adaptively attends to relevant SDMap skeletons and significantly improves performance. On the other hand, we exploit a masked autoencoder to capture the prior distribution of HDMap, which can serve as a refinement module to mitigate occlusions and artifacts. We benchmark on the nuScenes and Argoverse2 datasets. Through comprehensive experiments, we show that: (1) our SDMap prior can improve online map generation performance, using both rasterized (by up to $+18.73$ $\rm mIoU$) and vectorized (by up to $+8.50$ $\rm mAP$) output representations. (2) our HDMap prior can improve map perceptual metrics by up to $6.34\%$. (3) P-MapNet can be switched into different inference modes that covers different regions of the accuracy-efficiency trade-off landscape. (4) P-MapNet is a far-seeing solution that brings larger improvements on longer ranges. Codes and models are publicly available at https://jike5.github.io/P-MapNet.

==> pr.tex <==
Place Recongnition (PR) is crucial for the performance of a robot's navigation. A typical pipeline for the PR includes feature extraction, image retrieval and/or 2D-3D feature matching \cite{DBLP:journals/corr/abs-1911-11763} \cite{ sarlin2021back} \cite{7572201}. However, its high cost in terms of computation and memory footprint leaves room for improvement. PoseNet \cite{Kendall_2015_ICCV} proposes the method called absolute pose regression (APR) which first addresses this problem using a deep neural network.
% However, in practice, its localization accuracy is not yet comparable with structure-based ones. This is because the data sets for training regressors are often too small and lack variety in camera poses, therefore, a common view relationship between frames is enough to make the network converge.
Still, in large-scale scenes, it is difficult to cover the entire scene from one single perspective, so optimizing poses at any position is especially important. LENS \cite{DBLP:journals/corr/abs-2110-06558} has validated that introducing NeRF for data augmentation improves the localization accuracy. However, its training phase is still not memory-efficient. Direct-PoseNet \cite{DBLP:journals/corr/abs-2104-04073} and DFNet \cite{https://doi.org/10.48550/arxiv.2204.00559} deliver the state-of-the-art performances.

==> tables/mask_ratio.tex <==
\begin{table}[h]
  \caption{\textbf{Ablations about mask proportion.} We use different random mask ratios for pre-training, with higher mask ratios being harder for the reconstruction.
  }
  \begin{center}
  \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|ccc|c}
    \toprule
    Mask Proportion & Divider & Ped Crossing & Boundary & mIoU\\
    \midrule
    25\% & 64.8 & 51.4 & 67.6 & 61.27 \\
    50\% & \textbf{65.3} & {52.0} & \textbf{68.0} & \textbf{61.77} \\
    75\% & {64.7} & \textbf{52.1} & {67.7} & {61.50} \\
    \bottomrule
  \end{tabular}
  }
  \end{center}
  \label{tab:mask_ratio}
\end{table}
